Faa$T: A Transparent Auto-Scaling Cache for Serverless Applications

Function-as-a-Service (FaaS) has become an increasingly popular way for users to deploy their applications without the burden of managing the underlying infrastructure. However, existing FaaS platforms rely on remote storage to maintain state, limiting the set of applications that can be run efficiently. Recent caching work for FaaS platforms has tried to address this problem, but has fallen short: it disregards the widely different characteristics of FaaS applications, does not scale the cache based on data access patterns, or requires changes to applications. To address these limitations, we present Faa\$T, a transparent auto-scaling distributed cache for serverless applications. Each application gets its own Faa\$T cache. After a function executes and the application becomes inactive, the cache is unloaded from memory with the application. Upon reloading for the next invocation, Faa\$T pre-warms the cache with objects likely to be accessed. In addition to traditional compute-based scaling, Faa\$T scales based on working set and object sizes to manage cache space and I/O bandwidth. We motivate our design with a comprehensive study of data access patterns in a large-scale commercial FaaS provider. We implement Faa\$T for the provider's production FaaS platform. Our experiments show that Faa\$T can improve performance by up to 92% (57% on average) for challenging applications, and reduce cost for most users compared to state-of-the-art caching systems, i.e. the cost of having to stand up additional serverful resources.

==> fig-accessesperapp.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/characterization-accesses-per-app}
    \vspace{-.15in}
    \caption{CDF of the number of function invocations per unique
      blob by each application. 
      32\% of applications access the same blob in more than one invocation.
      11\% access the same block in more than 100 invocations.
    }
    \label{fig:characterization-accesses-per-app}
  \vspace{-.2in}
\end{figure}




==> fig-accessestime.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{figures/characterization-accessestime.png} %
  \vspace{-.15in}
  \caption{
    Coefficient of variation (CoV) of the inter-arrival time (IaT) and number of invocations for each blob accessed more than three times.
    A CoV of 1 indicates a Poisson arrival; closer to 0 is perfectly periodic; and larger than 1 indicates burstiness.
  }
  \label{fig:accesses-time}
  \vspace{-.2in}
\end{figure}


==> fig-blobsize.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{figures/characterization-blobsize}
  \vspace{-.15in}
  \caption{
    Distribution of the size of accessed blobs.
    80\% of accessed blobs are smaller than 12KB, and more than 25\% are smaller than 600 bytes.
  }
  \label{fig:characterization-blobsize}
  \vspace{-.1in}
\end{figure}



==> fig-compareall.tex <==
\begin{figure*}[t!]
  \centering
  \begin{subfigure}{0.3\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{figures/evaluation/alexnet_all.pdf}
    \caption{Inference with AlexNet}
    \label{fig:alexnet}
  \end{subfigure}
  \begin{subfigure}{0.3\textwidth}
    \includegraphics[width=1\textwidth]{figures/evaluation/squeezenet_all.pdf}
    \caption{Inference with SqueezeNet}
    \label{fig:squeezenet}
  \end{subfigure}
  \begin{subfigure}{0.3\textwidth}
    \includegraphics[width=1\textwidth]{figures/evaluation/infpipeline_all.pdf}
    \caption{AMBER Alert pipeline}
    \label{fig:infpipeline}
  \end{subfigure}
  \caption{
    Execution time for \faast for local hits, local misses, remote hits, and remote misses.
    Local miss is equivalent to Vanilla Azure Functions, and remote hit is equivalent to InfiniCache.
    For remote hits and misses, a total of two instances were used.
  }
  \label{fig:versus-all}
\end{figure*}


==> fig-consistency.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{figures/evaluation/consistency_box.pdf}
  \caption{
    Per-request latency for different write/read settings when summing to 1000 using a JupyterLess notebook with 5 instances sharing state.
    Each setting is abbreviated with its write, (mode), and read from Table~\ref{tab:consistency} (\eg, Storage Sync Storage becomes SSS).
    Performance is most variable when accesses are to remote storage, and least variable when accesses are to the local cache.
  }
  \label{fig:consistency}
\end{figure}


==> fig-consistent-hash.tex <==
\begin{figure}
  \centering
  \begin{subfigure}[t]{0.45\linewidth}
    \includegraphics[width=1\textwidth]{figures/faast_chbefore.pdf}
    \label{fig:consistenthashingbefore}
  \end{subfigure}
  \begin{subfigure}[t]{0.45\linewidth}
    \includegraphics[width=1\textwidth]{figures/faast_chafter.pdf}
    \label{fig:consistenthashingafter}
  \end{subfigure}
  \caption{
    \faast's consistent hashing with (a) three instances, and (b) two instances after one is unloaded.
    With four data objects and two instances, an average of two objects need to be remapped.
  }
  \label{fig:consistent-hash}
\end{figure}


==> fig-data-access.tex <==
\begin{figure*}[t]
  \centering
  \begin{subfigure}[t]{0.24\linewidth}
    \includegraphics[width=1\textwidth]{figures/faast_localhit.pdf}
    \caption{Local hit.}
    \label{fig:localhit}
  \end{subfigure}
  \begin{subfigure}[t]{0.24\linewidth}
    \includegraphics[width=1\textwidth]{figures/faast_localmiss.pdf}
    \caption{Local miss.}
    \label{fig:localmiss}
  \end{subfigure}
  \begin{subfigure}[t]{0.24\linewidth}
    \includegraphics[width=1\textwidth]{figures/faast_remotehit.pdf}
    \caption{Remote hit.}
    \label{fig:remotehit}
  \end{subfigure}
  \begin{subfigure}[t]{0.24\linewidth}
    \includegraphics[width=1\textwidth]{figures/faast_remotemiss.pdf}
    \caption{Remote miss.}
    \label{fig:remotemiss}
  \end{subfigure}
  \caption{
    Different cases for \faast reads.
    Solid lines indicate communication between the application, \faast instances, and remote storage.
    Dashed lines indicate data movement.
  }
  \label{fig:data-access}
  \vspace*{-.2in}
\end{figure*}


==> fig-numblobaccesses.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{figures/characterization-numblobaccesses.pdf}
  \caption{
    Distribution of accesses per blob for all functions that made at least one blob access (0.01\%).
    About 35\% of blobs are accessed more than once in a 24hr period.
  }
  \label{fig:characterization-numblobaccesses}
\end{figure}

